Post-Newtonian magnetohydrodynamics

In this paper, we derive the post-Newtonian equations of the ideal Magnetohydrodynamics. To do so, we use the modern approach to post-Newtonian theory, where the harmonic gauge is used instead of the standard post-Newtonian gauge, and find the post-Newtonian metric in the presence of the electromagnetic fields. We show that although the electric field does not contribute in the metric and curvature of the spacetime, the magnetic field appears in the time-time component of the metric. The appearance of the magnetic field, in principle, leads to new relativistic contributions to the magnetohydrodynamic governing equations. Therefore, using the post-Newtonian metric, we find the relativistic corrections to the magnetohydrodynamic equations up to the first post-Newtonian order. In addition, as usage of this derivation, we obtain a complete set of equations by which the behavior of a self-gravitating plasma can be determined in post-Newtonian gravity.

==> aliases.tex <==
\usepackage{xspace}

%  FORMATS
\newcommand{\dspaceon}{\renewcommand{\baselinestretch}{1.1}\large\normalsize}
\newcommand{\dspaceoff}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\footon}{\dspaceoff\footnotesize}
\newcommand{\bk}{\!\!\!\!}

% MATH
\newcommand{\mean}[1]{\ensuremath{\langle#1\rangle}}
\newcommand{\abs}[1]{\lvert#1\rvert} 
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\sub}[1]{\ensuremath{{_{\rm{#1}}}}}
\newcommand{\super}[1]{\ensuremath{{^{\rm{#1}}}}}
\newcommand{\rootn}{\ensuremath{\sqrt{n}}\xspace}

%  UNITS
\newcommand{\cps}{\,s$^{-1}$\xspace}
\newcommand{\un}[1]{\,\ensuremath{\rm{#1}}}
\newcommand{\as}{$^{\prime\prime}$\xspace}
\newcommand{\am}{$^{\prime}$\xspace}
\newcommand{\degrees}{$^{\circ}$}
\newcommand{\rsol}{\,$R_{\odot}$\xspace}
\newcommand{\lsol}{\,$L_{\odot}$\xspace}
\newcommand{\tsol}{\,$\tau_{\odot}$\xspace}
\newcommand{\msun}{\,$M_{\odot}$\xspace}
\newcommand{\msol}{\msun}
\newcommand{\lsun}{\,$L_{\odot}$\xspace}
\newcommand{\rsun}{\,$R_{\odot}$\xspace}
\newcommand{\msunperyear}{\msol\!$\rm yr^{-1}$\xspace}
\newcommand{\msolperyear}{\msunperyear}
\newcommand{\ergpersec}{\un{ergs\;s^{-1}}\xspace}
\newcommand{\ergpercmsec}{\un{ergs\,cm^{-2}\,s^{-1}}\xspace}
\newcommand{\percmsec}{\un{cm^{-2}\,s^{-1}}\xspace}
\newcommand{\percmsqrd}{\un{cm^{-2}}\xspace}
\newcommand{\phpercmseckev}{\un{ph\;cm^{-2}\,s^{-1}\,keV^{-1}}\xspace}
\newcommand{\phpercmsec}{\un{ph\;cm^{-2}\,s^{-1}}\xspace}
\newcommand{\rs}{\,$r_{\rm s}$\xspace}
\newcommand{\rlso}{\,$r_{\rm lso}$\xspace}
\newcommand{\rmso}{\,$r_{\rm mso}$\xspace}

%  INSTRUMENTS
\newcommand{\cgro}{{\em CGRO\/}\xspace}
\newcommand{\comptel}{{\small COMPTEL}\xspace}
\newcommand{\egret}{{\small EGRET}\xspace}
\newcommand{\integ}{{\sl INTEGRAL\/}\xspace}
\newcommand{\ibis}{{\small IBIS}\xspace}
\newcommand{\isgri}{{\small ISGRI}\xspace}
\newcommand{\picsit}{{\small PICSIT}\xspace}
\newcommand{\spi}{{\small SPI}\xspace}
\newcommand{\jemx}{{\small JEM-X}\xspace}
\newcommand{\omc}{{\small OMC}\xspace}
\newcommand{\hess}{{HESS}\xspace}

\newcommand{\fermi}{{\em Fermi}\xspace}
\newcommand{\uhuru}{{\em Uhuru}\xspace}
\newcommand{\ariel}{{\em Ariel\,V}\xspace}
\newcommand{\einstein}{{\em Einstein}\xspace}
\newcommand{\spacelab}{{\em Spacelab\,2}\xspace}
\newcommand{\xrt}{XRT\xspace}
\newcommand{\granat}{{\em Granat}\xspace}
\newcommand{\artp}{ART-P\xspace}
\newcommand{\sigm}{Sigma\xspace}
\newcommand{\ginga}{{\em Ginga}\xspace}
\newcommand{\asca}{{\em ASCA}\xspace}
\newcommand{\rosat}{{\em Rosat}\xspace}
\newcommand{\rxte}{{\small RXTE}\xspace}
\newcommand{\chandra}{{\em Chandra}\xspace}
\newcommand{\xmm}{{\em XMM-Newton}\xspace}
\newcommand{\suzaku}{{\em Suzaku}\xspace}
\newcommand{\epic}{{\small EPIC}\xspace}
\newcommand{\mos}{{\small MOS}\xspace}
\newcommand{\mosone}{{\small MOS1}\xspace}
\newcommand{\mostwo}{{\small MOS2}\xspace}
\newcommand{\pn}{{\small PN}\xspace}

\newcommand{\hst}{{\em HST\/}\xspace}
\newcommand{\hubble}{{\em Hubble Space Telescope\/}\xspace}
\newcommand{\keck}{{\it Keck}\xspace}
\newcommand{\cobe}{{\em COBE\/}\xspace}
\newcommand{\vla}{{\em VLA\/}\xspace}
\newcommand{\vlt}{{\em VLT\/}\xspace}


% SOURCES
\newcommand{\sgra}{Sgr\,A$^{*}$\xspace}
\newcommand{\sgraeast}{Sgr\,A\;East\xspace}
\newcommand{\sgrawest}{Sgr\;A\;West\xspace}
\newcommand{\igr}{IGR\,J17456--2901\xspace}
\newcommand{\ax}{AX\,J17456--2901\xspace}
\newcommand{\cxogc}{CXOGC\,J174540.0--290031\xspace}
\newcommand{\cxo}{\cxogc}
\newcommand{\xmmu}{XMMU\,J174554.4--285456\xspace}
\newcommand{\eg}{3EG\,J1746--2851\xspace}
\newcommand{\hessgc}{HESS\,J1745--290\xspace}


% WORDS
\newcommand{\afterTwoYears}{{\em A Persistent High-Energy Flux from the Heart of the Milky Way: INTEGRAL's View of the Galactic Center\/}\xspace}
\newcommand{\gammarays}{$\gamma$-rays\xspace}
\newcommand{\gammaray}{$\gamma$-ray\xspace}
\newcommand{\xray}{X-ray\xspace}
\newcommand{\xrays}{X-rays\xspace}
\newcommand{\fwhm}{FWHM\xspace}
\newcommand{\gti}{{\small GTI}\xspace}
\newcommand{\gtis}{{\small GTI}s\xspace}
\newcommand{\psla}{{\small PSLA}\xspace}
\newcommand{\arf}{{\small ARF}\xspace}
\newcommand{\arfs}{{\small ARF}s\xspace}
\newcommand{\rmf}{{\small RMF}\xspace}
\newcommand{\rmfs}{{\small RMF}s\xspace}
\newcommand{\pwn}{{\small PWN}\xspace}
\newcommand{\sn}{{\small SN}\xspace}
\newcommand{\snr}{{\small SNR}\xspace}
\newcommand{\snrs}{{\small SNR}s\xspace}
\newcommand{\gc}{{\small GC}\xspace}
\newcommand{\gcde}{{\small GCDE}\xspace}
\newcommand{\gd}{Galactic disk\xspace}
\newcommand{\gn}{{\small GN}\xspace}
\newcommand{\psf}{{\small PSF}\xspace}
\newcommand{\spsf}{{\small SPSF}\xspace}
\newcommand{\rms}{{\small RMS}\xspace}
\newcommand{\go}{{\small GO}\xspace}
\newcommand{\xspec}{{\small XSPEC}\xspace}
\newcommand{\glimpse}{{\small GLIMPSE}\xspace}
\newcommand{\ir}{{\small IR}\xspace}
\newcommand{\nir}{near-\ir}
\newcommand{\uv}{{\small UV}\xspace}
\newcommand{\ic}{{\small IC}\xspace}
\newcommand{\bh}{{\small BH}\xspace}
\newcommand{\osa}{{\small OSA}\xspace}
\newcommand{\sas}{{\small SAS}\xspace}
\newcommand{\isdc}{{\small ISDC}\xspace}
\newcommand{\ccd}{{\small CCD}\xspace}
\newcommand{\ccds}{{\small CCD}s\xspace}
\newcommand{\lmxb}{{\small LMXB}\xspace}
\newcommand{\lmxbs}{{\small LMXB}s\xspace}
\newcommand{\ism}{{\small ISM}\xspace}
\newcommand{\gmc}{{\small GMC}\xspace}
\newcommand{\gmcs}{{\small GMC}s\xspace}
\newcommand{\cmz}{{\small CMZ}\xspace}
\newcommand{\cnd}{{\small CND}\xspace}
\newcommand{\imf}{{\small IMF}\xspace}
\newcommand{\ura}{URA\xspace}
\newcommand{\mura}{MURA\xspace}
\newcommand{\og}{OG\xspace}
\newcommand{\ssc}{SSC\xspace}
\newcommand{\lso}{LSO\xspace}
\newcommand{\mso}{MSO\xspace}
\newcommand{\xrb}{XRB\xspace}
\newcommand{\xrbs}{XRBs\xspace}
\newcommand{\pdf}{{\small PDF\/}\xspace}
\newcommand{\cdf}{{\small CDF\/}\xspace}
\newcommand{\dof}{{\small DOF\/}\xspace}
\newcommand{\dft}{{\small DFT\/}\xspace}
\newcommand{\fft}{{\small FFT\/}\xspace}
\newcommand{\ifs}{{\small IFS\/}\xspace}
\newcommand{\psd}{{\small PSD\/}\xspace}
\newcommand{\pds}{{\small PDS\/}\xspace}


\newcommand{\hone}{H\,{\sc i\/}\xspace}
\newcommand{\htwo}{H\,{\sc ii\/}\xspace}
\newcommand{\neontwo}{Ne\,{\sc ii\/}\xspace}
\newcommand{\feone}{Fe\,{\sc i\/}\xspace}
\newcommand{\fetwentyfive}{Fe\,{\sc xxv\/}\xspace}
\newcommand{\fetwentysix}{Fe\,{\sc xxvi\/}\xspace}
\newcommand{\nione}{Ni\,{\sc i\/}\xspace}
\newcommand{\nitwentyseven}{Ni\,{\sc xxvii\/}\xspace}

